Polymorphic Endpoint Types for Copyless Message Passing

We present PolySing#, a calculus that models process interaction based on copyless message passing, in the style of Singularity OS. We equip the calculus with a type system that accommodates polymorphic endpoint types, which are a variant of polymorphic session types, and we show that well-typed processes are free from faults, leaks, and communication errors. The type system is essentially linear, although linearity alone may leave room for scenarios where well-typed processes leak memory. We identify a condition on endpoint types that prevents these leaks from occurring.

==> eptcsdata.tex <==
\providecommand{\firstpage}{52}
\providecommand{\publicationstatus}{Bliudze, S., Bruni, R., Carbone, M., Silva, A. (Eds.); ICE 2011\\
EPTCS 59, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.59.5}{10.4204/EPTCS.59.5}}

